Cell Detection by Functional Inverse Diffusion and Non-negative Group Sparsity$-$Part I: Modeling and Inverse Problems

In this two-part paper, we present a novel framework and methodology to analyze data from certain image-based biochemical assays, e.g., ELISPOT and Fluorospot assays. In this first part, we start by presenting a physical partial differential equations (PDE) model up to image acquisition for these biochemical assays. Then, we use the PDEs' Green function to derive a novel parametrization of the acquired images. This parametrization allows us to propose a functional optimization problem to address inverse diffusion. In particular, we propose a non-negative group-sparsity regularized optimization problem with the goal of localizing and characterizing the biological cells involved in the said assays. We continue by proposing a suitable discretization scheme that enables both the generation of synthetic data and implementable algorithms to address inverse diffusion. We end Part I by providing a preliminary comparison between the results of our methodology and an expert human labeler on real data. Part II is devoted to providing an accelerated proximal gradient algorithm to solve the proposed problem and to the empirical validation of our methodology.

==> figs/discretization_reg.tex <==
% Thought for use inside discretization_grid.tex only. Takes ``arguments'' from defined macros and
% plots the corresponding discretization region.	
	
	\pgfmathsetmacro{\mpo}{\m+1} \pgfmathsetmacro{\npo}{\n+1}
	% Draw square on xy plane
	\draw[dashed] (\xmin+\n*\xbynbins,0,\ymin+\m*\ybynbins) -- (\xmin+\npo*\xbynbins,0,\ymin+\m*\ybynbins) --
			(\xmin+\npo*\xbynbins,0,\ymin+\mpo*\ybynbins) -- (\xmin+\n*\xbynbins,0,\ymin+\mpo*\ybynbins) --
			(\xmin+\n*\xbynbins,0,\ymin+\m*\ybynbins);
	% Throw lines from the corners of the selected xy square
	\draw[thin,dashed,gray!60] (\xmin+\n*\xbynbins,0,\ymin+\m*\ybynbins) -- (\xmin+\n*\xbynbins,\sigmaxn,\ymin+\m*\ybynbins);
	\draw[thin,dashed,gray!60] (\xmin+\npo*\xbynbins,0,\ymin+\m*\ybynbins) -- (\xmin+\npo*\xbynbins,\sigmaxn,\ymin+\m*\ybynbins);
	\draw[thin,dashed,gray!60] (\xmin+\npo*\xbynbins,0,\ymin+\mpo*\ybynbins) -- (\xmin+\npo*\xbynbins,\sigmaxn,\ymin+\mpo*\ybynbins);
	\draw[thin,dashed,gray!60] (\xmin+\n*\xbynbins,0,\ymin+\mpo*\ybynbins) -- (\xmin+\n*\xbynbins,\sigmaxn,\ymin+\mpo*\ybynbins);
	% Draw selected segment on \sigma dimension
	\draw[dashed] (.25*\xdist,\sigselmin*\lofsig,0) -- (.25*\xdist,\sigselmax*\lofsig,0);
	% Throw lines from the corners of the selected segment
	\draw[thin,dashed,gray!60] (.25*\xdist,\sigselmin*\lofsig,0) -- (\xmax,\sigselmin*\lofsig,0);
	\draw[thin,dashed,gray!60] (.25*\xdist,\sigselmax*\lofsig,0) -- (\xmax,\sigselmax*\lofsig,0);
	% Draw selected segment on \sigma-x plane
	\draw[dashed] (\xmin+\n*\xbynbins,\sigselmin*\lofsig,0) -- (\xmin+\npo*\xbynbins,\sigselmin*\lofsig,0) --
			(\xmin+\npo*\xbynbins,\sigselmax*\lofsig,0) -- (\xmin+\n*\xbynbins,\sigselmax*\lofsig,0) --
			(\xmin+\n*\xbynbins,\sigselmin*\lofsig,0);
	% Throw lines upwards from the corners of the selected \sigma-x square
	\draw[thin,dashed,gray!60] (\xmin+\n*\xbynbins,\sigselmin*\lofsig,0) -- (\xmin+\n*\xbynbins,\sigselmin*\lofsig,\ymax);
	\draw[thin,dashed,gray!60] (\xmin+\npo*\xbynbins,\sigselmin*\lofsig,0) -- (\xmin+\npo*\xbynbins,\sigselmin*\lofsig,\ymax);
	\draw[thin,dashed,gray!60] (\xmin+\npo*\xbynbins,\sigselmax*\lofsig,0) -- (\xmin+\npo*\xbynbins,\sigselmax*\lofsig,\ymax);
	\draw[thin,dashed,gray!60] (\xmin+\n*\xbynbins,\sigselmax*\lofsig,0) -- (\xmin+\n*\xbynbins,\sigselmax*\lofsig,\ymax);
	% Highlight selected discretization region	
		% Foreground cube layer
		\draw[thick] (\xmin+\n*\xbynbins,\sigselmin*\lofsig,\ymin+\m*\ybynbins) --
						(\xmin+\n*\xbynbins,\sigselmin*\lofsig,\ymin+\mpo*\ybynbins) --
						(\xmin+\n*\xbynbins,\sigselmax*\lofsig,\ymin+\mpo*\ybynbins) --
						(\xmin+\n*\xbynbins,\sigselmax*\lofsig,\ymin+\m*\ybynbins) -- cycle;
		% Unseen cube lines
		\draw[thick,dashed] (\xmin+\n*\xbynbins,\sigselmin*\lofsig,\ymin+\m*\ybynbins) --
								(\xmin+\npo*\xbynbins,\sigselmin*\lofsig,\ymin+\m*\ybynbins) --
								(\xmin+\npo*\xbynbins,\sigselmax*\lofsig,\ymin+\m*\ybynbins);
		\draw[thick,dashed] (\xmin+\npo*\xbynbins,\sigselmin*\lofsig,\ymin+\m*\ybynbins) --
								(\xmin+\npo*\xbynbins,\sigselmin*\lofsig,\ymin+\mpo*\ybynbins);
		% Lid cube layer
		\draw[thick] (\xmin+\n*\xbynbins,\sigselmin*\lofsig,\ymin+\mpo*\ybynbins) --
							(\xmin+\npo*\xbynbins,\sigselmin*\lofsig,\ymin+\mpo*\ybynbins) --
							(\xmin+\npo*\xbynbins,\sigselmax*\lofsig,\ymin+\mpo*\ybynbins) --
							(\xmin+\n*\xbynbins,\sigselmax*\lofsig,\ymin+\mpo*\ybynbins) -- cycle;
		% Remaining cube lines
		\draw[thick] (\xmin+\npo*\xbynbins,\sigselmax*\lofsig,\ymin+\mpo*\ybynbins) --
							(\xmin+\npo*\xbynbins,\sigselmax*\lofsig,\ymin+\m*\ybynbins) --
							(\xmin+\n*\xbynbins,\sigselmax*\lofsig,\ymin+\m*\ybynbins);
